Magnus and Dyson Series for Master Integrals

We elaborate on the method of differential equations for evaluating Feynman integrals. We focus on systems of equations for master integrals having a linear dependence on the dimensional parameter. For these systems we identify the criteria to bring them in a canonical form, recently identified by Henn, where the dependence of the dimensional parameter is disentangled from the kinematics. The determination of the transformation and the computation of the solution are obtained by using Magnus and Dyson series expansion. We apply the method to planar and non-planar two-loop QED vertex diagrams for massive fermions, and to non-planar two-loop integrals contributing to 2 -> 2 scattering of massless particles. The extension to systems which are polynomial in the dimensional parameter is discussed as well.

==> PICTURES/Bhabha/aa.tex <==
\unitlength=1bp%

\begin{feynartspicture}(432,504)(1,1)

\FADiagram{}
\FAProp(0.,15.)(4.,10.)(0.,){Straight}{1}
\FALabel(1.26965,12.0117)[tr]{$e$}
\FAProp(0.,5.)(4.,10.)(0.,){Straight}{-1}
\FALabel(2.73035,7.01172)[tl]{$e$}
\FAProp(20.,15.)(16.,13.5)(0.,){Straight}{-1}
\FALabel(17.4558,15.2213)[b]{$e$}
\FAProp(20.,5.)(16.,6.5)(0.,){Straight}{1}
\FALabel(17.4558,4.77869)[t]{$e$}
\FAProp(4.,10.)(10.,10.)(0.,){Sine}{0}
\FALabel(7.,11.07)[b]{$\gamma$}
\FAProp(16.,13.5)(16.,6.5)(0.,){Sine}{0}
\FALabel(17.07,10.)[l]{$\gamma$}
\FAProp(16.,13.5)(10.,10.)(0.,){Straight}{-1}
\FALabel(12.699,12.6089)[br]{$e$}
\FAProp(16.,6.5)(10.,10.)(0.,){Straight}{1}
\FALabel(12.699,7.39114)[tr]{$e$}
\FAVert(4.,10.){0}
\FAVert(16.,13.5){0}
\FAVert(16.,6.5){0}
\FAVert(10.,10.){0}
\end{feynartspicture}

\begin{feynartspicture}(432,504)(1,1)

\FADiagram{}
\FAProp(0.,15.)(4.,13.5)(0.,){Straight}{1}
\FALabel(2.54424,15.2213)[b]{$e$}
\FAProp(0.,5.)(4.,6.5)(0.,){Straight}{-1}
\FALabel(2.54424,4.77869)[t]{$e$}
\FAProp(20.,15.)(16.,10.)(0.,){Straight}{-1}
\FALabel(17.2697,12.9883)[br]{$e$}
\FAProp(20.,5.)(16.,10.)(0.,){Straight}{1}
\FALabel(18.7303,7.98828)[bl]{$e$}
\FAProp(16.,10.)(10.,10.)(0.,){Sine}{0}
\FALabel(13.,8.93)[t]{$\gamma$}
\FAProp(4.,13.5)(4.,6.5)(0.,){Sine}{0}
\FALabel(2.93,10.)[r]{$\gamma$}
\FAProp(4.,13.5)(10.,10.)(0.,){Straight}{1}
\FALabel(7.301,12.6089)[bl]{$e$}
\FAProp(4.,6.5)(10.,10.)(0.,){Straight}{-1}
\FALabel(7.301,7.39114)[tl]{$e$}
\FAVert(4.,13.5){0}
\FAVert(4.,6.5){0}
\FAVert(16.,10.){0}
\FAVert(10.,10.){0}
\end{feynartspicture}

\begin{feynartspicture}(432,504)(1,1)

\FADiagram{}
\FAProp(0.,15.)(6.5,13.5)(0.,){Straight}{1}
\FALabel(3.59853,15.2803)[b]{$e$}
\FAProp(0.,5.)(6.5,6.5)(0.,){Straight}{-1}
\FALabel(3.59853,4.71969)[t]{$e$}
\FAProp(20.,15.)(13.5,13.5)(0.,){Straight}{-1}
\FALabel(16.4015,15.2803)[b]{$e$}
\FAProp(20.,5.)(13.5,6.5)(0.,){Straight}{1}
\FALabel(16.4015,4.71969)[t]{$e$}
\FAProp(6.5,13.5)(6.5,6.5)(0.,){Straight}{1}
\FALabel(5.43,10.)[r]{$e$}
\FAProp(6.5,13.5)(13.5,13.5)(0.,){Sine}{0}
\FALabel(10.,14.57)[b]{$\gamma$}
\FAProp(6.5,6.5)(13.5,6.5)(0.,){Sine}{0}
\FALabel(10.,5.43)[t]{$\gamma$}
\FAProp(13.5,13.5)(13.5,6.5)(0.,){Straight}{-1}
\FALabel(14.57,10.)[l]{$e$}
\FAVert(6.5,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
\end{feynartspicture}

\begin{feynartspicture}(432,504)(1,1)

\FADiagram{}
\FAProp(0.,15.)(6.5,13.5)(0.,){Straight}{1}
\FALabel(3.59853,15.2803)[b]{$e$}
\FAProp(0.,5.)(6.5,6.5)(0.,){Straight}{-1}
\FALabel(3.59853,4.71969)[t]{$e$}
\FAProp(20.,15.)(13.5,13.5)(0.,){Straight}{-1}
\FALabel(16.4015,15.2803)[b]{$e$}
\FAProp(20.,5.)(13.5,6.5)(0.,){Straight}{1}
\FALabel(16.4015,4.71969)[t]{$e$}
\FAProp(6.5,13.5)(6.5,6.5)(0.,){Sine}{0}
\FALabel(5.43,10.)[r]{$\gamma$}
\FAProp(6.5,13.5)(13.5,13.5)(0.,){Straight}{1}
\FALabel(10.,14.57)[b]{$e$}
\FAProp(6.5,6.5)(13.5,6.5)(0.,){Straight}{-1}
\FALabel(10.,5.43)[t]{$e$}
\FAProp(13.5,13.5)(13.5,6.5)(0.,){Sine}{0}
\FALabel(14.57,10.)[l]{$\gamma$}
\FAVert(6.5,13.5){0}
\FAVert(6.5,6.5){0}
\FAVert(13.5,13.5){0}
\FAVert(13.5,6.5){0}
\end{feynartspicture}

\begin{feynartspicture}(432,504)(1,1)

\FADiagram{}
\FAProp(0.,15.)(3.,10.)(0.,){Straight}{1}
\FALabel(0.650886,12.1825)[tr]{$e$}
\FAProp(0.,5.)(3.,10.)(0.,){Straight}{-1}
\FALabel(2.34911,7.18253)[tl]{$e$}
\FAProp(20.,15.)(17.,10.)(0.,){Straight}{-1}
\FALabel(17.6509,12.8175)[br]{$e$}
\FAProp(20.,5.)(17.,10.)(0.,){Straight}{1}
\FALabel(19.3491,7.81747)[bl]{$e$}
\FAProp(3.,10.)(7.,10.)(0.,){Sine}{0}
\FALabel(5.,11.07)[b]{$\gamma$}
\FAProp(17.,10.)(13.,10.)(0.,){Sine}{0}
\FALabel(15.,8.93)[t]{$\gamma$}
\FAProp(7.,10.)(13.,10.)(0.8,){Straight}{-1}
\FALabel(10.,6.53)[t]{$e$}
\FAProp(7.,10.)(13.,10.)(-0.8,){Straight}{1}
\FALabel(10.,13.47)[b]{$e$}
\FAVert(3.,10.){0}
\FAVert(17.,10.){0}
\FAVert(7.,10.){0}
\FAVert(13.,10.){0}
\end{feynartspicture}



==> PICTURES/Box2C/Diagrams1.tex <==
\unitlength=0.3bp%
\hspace{5cm}
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(5.5,13.5)(0.,){Straight}{0}
\FAProp(0.,5.)(5.5,6.5)(0.,){Straight}{0}
\FAProp(20.,15.)(14.5,13.5)(0.,){Straight}{0}
\FAProp(20.,5.)(14.5,6.5)(0.,){Straight}{0}
%
\FAProp(5.5,13.5)(5.5,6.5)(0.,){Straight}{-1}
\FALabel(3.7,10.)[]{\scriptsize $k_1$}
\FAProp(5.5,13.5)(14.5,13.5)(0.,){Straight}{0}
\FAProp(5.5,6.5)(14.5,6.5)(0.,){Straight}{0}
%\FAProp(14.5,13.5)(14.5,6.5)(0.,){Straight}{0}
%
\FAProp(14.5,13.5)(12.25, 10)(0.,){Straight}{0}
\FAProp(12.25, 10)(10.,6.5)(0.,){Straight}{0}
\FAProp(14.5,6.5)(10.,13.5)(0.,){Straight}{0}
\FALabel(18.6, 11.75)[]{\scriptsize $k_1-k_2$}
%
\FALabel(4.2,16.4)[]{\small $p_1$}
\FALabel(4.2,3.6)[]{\small $p_3$}
\FALabel(15.8,16.4)[]{\small $p_4$}
\FALabel(15.8,3.6)[]{\small $p_2$}
%\FALabel(10.,0.)[]{$\top{g}(s,t)$}
\end{feynartspicture}
\hspace{5cm}


==> PICTURES/Box2C/Masters1.tex <==
\unitlength=0.25bp%
\hspace{0.3cm}
% T1
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,10.)(6.,10.)(0.,){Straight}{0}
%\FALabel(3.,8.93)[t]{$g$}
\FAProp(20.,10.)(14.,10.)(0.,){Straight}{0}
%\FALabel(17.,11.07)[b]{$g$}
\FAProp(14.,10.)(6.,10.)(-1.,){Straight}{0}
%\FALabel(10.,4.93)[t]{$g$}
\FAProp(14.,10.)(6.,10.)(0.,){Straight}{0}
\FAVert(10.,10.){0}
\FAVert(10.,6.){0}
%\FALabel(10.,8.23)[t]{$g$}
\FAProp(14.,10.)(6.,10.)(1.,){Straight}{0}
%\FALabel(10.,15.07)[b]{\small $g$}
%\FAVert(14.,10.){0}
%\FAVert(6.,10.){0}
\FALabel(2.,8.93)[t]{\small $p_{12}$}
\FALabel(10.,0.)[]{$\top{a}(s)$}
\end{feynartspicture}
\hspace{0.3cm}
%
% T2
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.,15.)(0.,){Straight}{0}
%\FALabel(3.,16.77)[b]{$g$}
\FAProp(0.,5.)(6.,5.)(0.,){Straight}{0}
%\FALabel(3.,3.93)[t]{$g$}
\FAProp(20.,10.)(14.5,10.)(0.,){Straight}{0}
%\FALabel(17.25,8.23)[t]{$g$}
\FAProp(14.5,10.)(6.,5.)(0.,){Straight}{0}
%\FALabel(10.9108,6.04065)[tl]{$g$}
\FAProp(14.5,10.)(6.,15.)(0.,){Straight}{0}
%\FALabel(10.5559,13.356)[bl]{$g$}
\FAProp(6.,5.)(6.,15.)(-0.4,){Straight}{0}
%\FALabel(2.93,10.)[r]{$g$}
\FAProp(6.,5.)(6.,15.)(0.4,){Straight}{0}
\FAVert(8.,10.){0}
%\FALabel(9.07,10.)[l]{$g$}
%\FAVert(14.5,10.){0}
%\FAVert(6.,5.){0}
%\FAVert(6.,15.){0}
\FALabel(2.5,16.77)[b]{\small $p_1$}
\FALabel(2.5,6.77)[b]{\small $p_2$}
\FALabel(10.,0.)[]{$\top{b}(s)$}
\end{feynartspicture}
%
% T3
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.5,13.5)(0.,){Straight}{0}
%\FALabel(3.75593,15.9624)[b]{$g$}
\FAProp(0.,5.)(6.5,6.5)(0.,){Straight}{0}
%\FALabel(3.59853,4.71969)[t]{$g$}
\FAProp(20.,15.)(13.5,13.5)(0.,){Straight}{0}
%\FALabel(16.4015,15.2803)[b]{$g$}
\FAProp(20.,5.)(13.5,6.5)(0.,){Straight}{0}
%\FALabel(16.2441,4.03762)[t]{$g$}
\FAProp(6.5,13.5)(6.5,6.5)(0.,){Straight}{0}
%\FALabel(5.43,10.)[r]{$g$}
\FAProp(6.5,13.5)(13.5,13.5)(0.,){Straight}{0}
%\FALabel(10.,15.27)[b]{$g$}
\FAProp(6.5,6.5)(13.5,6.5)(0.,){Straight}{0}
%\FALabel(10.,5.43)[t]{$g$}
\FAProp(13.5,13.5)(13.5,6.5)(0.4,){Straight}{0}
\FAProp(13.5,13.5)(13.5,6.5)(-0.4,){Straight}{0}
\FAVert(14.9,10.0){0}
%\FALabel(15.27,10.)[l]{$g$}
%\FAVert(6.5,13.5){0}
%\FAVert(6.5,6.5){0}
%\FAVert(13.5,13.5){0}
%\FAVert(13.5,6.5){0}
\FALabel(4.2,16.4)[]{\small $p_1$}
\FALabel(4.2,3.6)[]{\small $p_4$}
\FALabel(15.8,16.4)[]{\small $p_3$}
\FALabel(15.8,3.6)[]{\small $p_2$}
\FALabel(10.,0.)[]{$\top{c}(s,t)$}
\end{feynartspicture}
\hspace{0.3cm}
%
% T4
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(6.5,13.5)(0.,){Straight}{0}
%\FALabel(3.75593,15.9624)[b]{$g$}
\FAProp(0.,5.)(6.5,6.5)(0.,){Straight}{0}
%\FALabel(3.59853,4.71969)[t]{$g$}
\FAProp(20.,15.)(13.5,13.5)(0.,){Straight}{0}
%\FALabel(16.4015,15.2803)[b]{$g$}
\FAProp(20.,5.)(13.5,6.5)(0.,){Straight}{0}
%\FALabel(16.2441,4.03762)[t]{$g$}
\FAProp(6.5,13.5)(6.5,6.5)(0.,){Straight}{0}
%\FALabel(5.43,10.)[r]{$g$}
\FAProp(6.5,13.5)(13.5,13.5)(0.,){Straight}{0}
%\FALabel(10.,15.27)[b]{$g$}
\FAProp(6.5,6.5)(13.5,6.5)(0.,){Straight}{0}
%\FALabel(10.,5.43)[t]{$g$}
\FAProp(13.5,13.5)(13.5,6.5)(0.,){Straight}{0}
%\FALabel(15.27,10.)[l]{$g$}
\FAProp(6.5,6.5)(13.5,13.5)(0.,){Straight}{0}
%\FAVert(6.5,13.5){0}
%\FAVert(6.5,6.5){0}
%\FAVert(13.5,13.5){0}
%\FAVert(13.5,6.5){0}
\FALabel(4.2,16.4)[]{\small $p_1$}
\FALabel(4.2,3.6)[]{\small $p_2$}
\FALabel(15.8,16.4)[]{\small $p_3$}
\FALabel(15.8,3.6)[]{\small $p_4$}
\FALabel(10.,0.)[]{$\top{d}(s,t)$}
\end{feynartspicture}
\hspace{0.3cm}
%
% T5
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(5.,15.)(0.,){Straight}{0}
%\FALabel(2.5,16.77)[b]{$g$}
\FAProp(0.,5.)(5.,5.)(0.,){Straight}{0}
%\FALabel(2.5,3.93)[t]{$g$}
\FAProp(20.,10.)(14.5,10.)(0.,){Straight}{0}
%\FALabel(17.25,8.23)[t]{$g$}
\FAProp(5.,15.)(9.,7.1)(0.,){Straight}{0}
%\FALabel(3.93,10.)[r]{$g$}
\FAProp(9.,12.95)(5.,15.)(0.,){Straight}{0}
%\FALabel(7.22694,14.8744)[bl]{$g$}
\FAProp(9.,12.95)(14.5,10.)(0.,){Straight}{0}
%\FALabel(11.4974,10.5891)[tr]{$g$}
\FAProp(5.,5.)(9.,12.95)(0.,){Straight}{0}
%\FALabel(10.07,10.025)[l]{$g$}
\FAProp(9.,7.1)(5.,5.)(0.,){Straight}{0}
%\FALabel(7.56588,4.53785)[tl]{$g$}
\FAProp(9.,7.1)(14.5,10.)(0.,){Straight}{0}
%\FALabel(11.9929,7.65892)[tl]{$g$}
%\FAVert(9.,7.1){0}
%\FAVert(9.,12.95){0}
%\FAVert(5.,15.){0}
%\FAVert(5.,5.){0}
%\FAVert(14.5,10.){0}
\FALabel(2.5,16.77)[b]{\small $p_1$}
\FALabel(2.5,6.77)[b]{\small $p_2$}
\FALabel(10.,0.)[]{$\top{e}(s)$}
\end{feynartspicture}
\hspace{0.3cm}
%
% T6
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(5.5,13.5)(0.,){Straight}{0}
\FAProp(0.,5.)(5.5,6.5)(0.,){Straight}{0}
\FAProp(20.,15.)(14.5,13.5)(0.,){Straight}{0}
\FAProp(20.,5.)(14.5,6.5)(0.,){Straight}{0}
%
\FAProp(5.5,13.5)(5.5,6.5)(0.,){Straight}{0}
\FAProp(5.5,13.5)(14.5,13.5)(0.,){Straight}{0}
\FAProp(5.5,6.5)(14.5,6.5)(0.,){Straight}{0}
%\FAProp(14.5,13.5)(14.5,6.5)(0.,){Straight}{0}
%
\FAProp(14.5,13.5)(10.,6.5)(0.,){Straight}{0}
\FAProp(14.5,6.5)(10.,13.5)(0.,){Straight}{0}
%
\FALabel(4.2,16.4)[]{\small $p_1$}
\FALabel(4.2,3.6)[]{\small $p_4$}
\FALabel(15.8,16.4)[]{\small $p_2$}
\FALabel(15.8,3.6)[]{\small $p_3$}
\FALabel(10.,0.)[]{$\top{f}(s,t)$}
\end{feynartspicture}
\hspace{0.3cm}
%
% T7
% T6
\begin{feynartspicture}(300,300)(1,1)
\FADiagram{}
\FAProp(0.,15.)(5.5,13.5)(0.,){Straight}{0}
\FAProp(0.,5.)(5.5,6.5)(0.,){Straight}{0}
\FAProp(20.,15.)(14.5,13.5)(0.,){Straight}{0}
\FAProp(20.,5.)(14.5,6.5)(0.,){Straight}{0}
%
\FAProp(5.5,13.5)(5.5,6.5)(0.,){Straight}{0}
\FAProp(5.5,13.5)(14.5,13.5)(0.,){Straight}{0}
\FAProp(5.5,6.5)(14.5,6.5)(0.,){Straight}{0}
%\FAProp(14.5,13.5)(14.5,6.5)(0.,){Straight}{0}
%
\FAProp(14.5,13.5)(10.,6.5)(0.,){Straight}{0}
\FAProp(14.5,6.5)(10.,13.5)(0.,){Straight}{0}
%
\FALabel(4.2,16.4)[]{\small $p_1$}
\FALabel(4.2,3.6)[]{\small $p_4$}
\FALabel(15.8,16.4)[]{\small $p_2$}
\FALabel(15.8,3.6)[]{\small $p_3$}
\FALabel(22.,10.)[]{\scriptsize $[(k_2+p_1)^2]$}
\FALabel(10.,0.)[]{$\top{g}(s,t)$}
\end{feynartspicture}
\hspace{0.3cm}
%
%
%
%
%
% BOX 1 LOOP
%
%\begin{feynartspicture}(300,300)(1,1)
%\FADiagram{}
%\FAProp(0.,15.)(6.5,13.5)(0.,){Straight}{0}
%%\FALabel(3.75593,15.9624)[b]{$g$}
%\FAProp(0.,5.)(6.5,6.5)(0.,){Straight}{0}
%%\FALabel(3.59853,4.71969)[t]{$g$}
%\FAProp(20.,15.)(13.5,13.5)(0.,){Straight}{0}
%%\FALabel(16.4015,15.2803)[b]{$g$}
%\FAProp(20.,5.)(13.5,6.5)(0.,){Straight}{0}
%%\FALabel(16.2441,4.03762)[t]{$g$}
%\FAProp(6.5,13.5)(6.5,6.5)(0.,){Straight}{0}
%%\FALabel(5.43,10.)[r]{$g$}
%\FAProp(6.5,13.5)(13.5,13.5)(0.,){Straight}{0}
%%\FALabel(10.,15.27)[b]{$g$}
%\FAProp(6.5,6.5)(13.5,6.5)(0.,){Straight}{0}
%%\FALabel(10.,5.43)[t]{$g$}
%\FAProp(13.5,13.5)(13.5,6.5)(0.,){Straight}{0}
%%\FALabel(15.27,10.)[l]{$g$}
%%\FAVert(6.5,13.5){0}
%%\FAVert(6.5,6.5){0}
%%\FAVert(13.5,13.5){0}
%%\FAVert(13.5,6.5){0}
%\FALabel(4.2,16.4)[]{\small $p_1$}
%\FALabel(4.2,3.6)[]{\small $p_4$}
%\FALabel(15.8,16.4)[]{\small $p_3$}
%\FALabel(15.8,3.6)[]{\small $p_2$}
%\FALabel(10.,0.)[]{$\top{xx}$}
%\end{feynartspicture}


